Empirical Guidelines for Deploying LLMs onto Resource-constrained Edge Devices

The scaling laws have become the de facto guidelines for designing large language models (LLMs), but they were studied under the assumption of unlimited computing resources for both training and inference. As LLMs are increasingly used as personalized intelligent assistants, their customization (i.e., learning through fine-tuning) and deployment onto resource-constrained edge devices will become more and more prevalent. An urging but open question is how a resource-constrained computing environment would affect the design choices for a personalized LLM. We study this problem empirically in this work. In particular, we consider the tradeoffs among a number of key design factors and their intertwined impacts on learning efficiency and accuracy. The factors include the learning methods for LLM customization, the amount of personalized data used for learning customization, the types and sizes of LLMs, the compression methods of LLMs, the amount of time afforded to learn, and the difficulty levels of the target use cases. Through extensive experimentation and benchmarking, we draw a number of surprisingly insightful guidelines for deploying LLMs onto resource-constrained devices. For example, an optimal choice between parameter learning and RAG may vary depending on the difficulty of the downstream task, the longer fine-tuning time does not necessarily help the model, and a compressed LLM may be a better choice than an uncompressed LLM to learn from limited personalized data.

==> 2_related.tex <==
\section{Background: Running LLMs on Edge Devices}
\label{sec:related}

Running an LLM on an edge device first requires loading the model weights into dynamic random-access memory (DRAM or RAM), where model training and inference can be performed based on the CPU or GPU. The RAM size on edge devices commonly ranges from 4G to 16G, as explained in Appendix~\ref{subsec:Edge_Device_Constraints}, thereby limiting the model weights. 
For a loaded edge LLM, its training can consume much more RAM than its inference does, risking exceeding the total available RAM.
During training, data are moved from disk to RAM. Compared to the time cost of gradient calculation, the cost of moving data can be relatively negligible. Given an edge device, the speed of learning (gradient calculation) can vary across different models. In our work, we use \textbf{throughput}, which is the amount of data a model can process in one hour, to measure the data a model can learn on some device. This is because LLM parameter learning on edge devices is more time-sensitive, and we need a uniform standard to measure the learning efficiency of each model. In the following, we use \textbf{normalized data size (NDS)} from 1 to 8 to represent the amount of data that a model can process within 1 to 8 hours. The detailed data size for each selected model to be trained per hour can be found in Table ~\ref{tab:model_data} in Appendix~\ref{subsec:profiling_LLMs_details}. 

\label{subsec:main_profiling}



==> 3_method.tex <==
\section{Preparation for Evaluation}
\label{sec:evaluation}

\subsection{Background: Running LLMs on Edge Devices}
\label{subsec:main_profiling}
% \label{sec:related}
In this paper, we use a range of common edge devices to profile the performance of LLMs running on them, as summarized in Appendix~\ref{subsec:Edge_Device_Constraints}. Running an LLM on an edge device requires loading the model weights into random-access memory (RAM) of edge CPUs or edge GPUs, where model fine-tuning (or equivalently referred to as training in this paper) and inference can be performed. The RAM size on these devices commonly ranges from 4G to 16G, thereby limiting the size of model weights. Note that the 
RAM capacity constraint applies to both training and inference, and the former is usually the bottleneck 
as training consumes more memory than inference 
does. In addition, LLM parameter learning on edge devices is time-sensitive, and the training time is affected by both the edge device's hardware computation density (which depends on the hardware architecture as well as clock frequency), and the model complexity. 
To rule out the impact of pure hardware factor, the training times reported in this paper are all scaled as if each device were running at 1.5 TFLOPS (corresponding to Apple A14 GPU), and they range from one to eight hours. Note that in the same training time, different models are able to process different amounts of data, which is shown in detail in Table~\ref{tab:model_data} in Appendix~\ref{subsec:profiling_LLMs_details}. 

\subsection{Data}
\label{subsec:data_preparation}
To investigate the customization of edge LLMs for each specific user, we concentrate on two task types: content classification and summarization. The edge LLMs should learn from the user history data and generate content to better adapt to the user's expectations. Hence, we use the datasets specifically designed to evaluate the LLM's personalization capabilities. Detailed reasons to use these datasets can be found in Appendix ~\ref{subsec:llm_evaluation}. The detailed dataset structures and their prompt format can be found in Appendix~\ref{subsec:Datasets}. We prepare the data for our edge LLM evaluation from two perspectives: user-level and task-level.

\textbf{User-level}: 
Each dataset contains many users, and each user has many samples of user history data and user query data. One sample of user history data and user query data are shown in Table~\ref{tab:table_lamp_profile_data} and in Table~\ref{tab:table_lamp_prompt} in Appendix ~\ref{subsec:Datasets}. 
In terms of generalization, we randomly select 100 users and calculate the average performance of edge LLMs over the 100 users in our evaluation.

\textbf{Task-level}: 
When evaluating various edge LLMs under multiple datasets (tasks), the difficulty of each task can be a latent factor impacting our evaluation \cite{ge2024openagi}. Within the same dataset, we assume that utterances have similar levels of difficulty \cite{wen2022empirical}. However, difficulties may vary across datasets, which is a non-negligible factor that requires attention. 
% When the LaMP datasets were proposed, zero-shot personalized results \cite{salemi2023lamp} using GPT-3.5 were provided to give a brief idea of how a well-performing LLM can perform on each dataset. 
Zero-shot learning can be used to measure the difficulty of a provided dataset on a well-performing pre-trained model \cite{liusie2024llm}. 
Therefore, we select GPT-4 \cite{achiam2023gpt}, Claude 3 Opus \cite{kevian2024capabilities}, Gemini 1.0 Pro \cite{team2023gemini}, and Llama 3 70B \cite{meta_llama3} to measure their performance on the testing data we choose from each dataset, and summarize the results in Table \ref{tab:lamp_difficulties}. For classification tasks, since each task has a different number of options, we consider a fairer assessment method similar to \cite{yin2024pruning}, where they normalize the accuracy with respect to human expert performance. However, since we could not get objective human performance on these datasets, we take an alternative approach by dividing the actual accuracy obtained from LLMs with the accuracy from random guessing, which we refer to as ``normalized accuracy'' in the table. Mathematically, the normalized accuracy is computed as $\frac{\text{accuracy}}{1/{\text{No. choices}}}$. For the summarization task, the normalized accuracy is the same as the accuracy. For the same type of task, the normalized accuracy can represent the difficulty of the task, where the higher the value, the easier the task is. Through our examination, the normalized accuracy for classification datasets are: LaMP-1 with 0.995, LaMP-2 with 5.157, and LaMP-3 with 3.236; the normalized accuracy for summarization datasets are: LaMP-4 with 0.1460, LaMP-5 with 0.3123, LaMP-6 with 0.3475, and LaMP-7 with 0.2385. The detailed results of each dataset in each cloud-based LLM can be found in Appendix~\ref{subsec:task_difficulty}. 


\subsection{Learning Methods}
\label{subsec:learning_methods}
% \zyan{[I want to delete some words, but haven't found a way yet.]}
There are two learning methods for edge LLM customization: parameter-efficient fine-tuning (PEFT) \cite{hu2023llm} and retrieval-augmented generation (RAG) \cite{chen2024benchmarking}. While both in general can improve the cloud-based LLM performance \cite{lakatos2024investigating}, the performance can fluctuate given different settings in different datasets. It is important to investigate whether similar situations exist on edge LLMs. 

\textbf{PEFT}: Compared to various PEFT implementations, low-rank adaption (LoRA) has demonstrated promising capabilities \cite{hu2021lora} in fine-tuning a wide range of LLMs and significantly improving their performance via updating a small portion of trainable parameters. The two hyperparameters \textit{rank} and \textit{alpha} can mostly impact the LoRA-tuning model performance \cite{lee2023platypus}. Hence, we set all other hyperparameters to default, as described in Appendix~\ref{subsec:Experimental_Settings}, and explore a wide range of rank and alpha value combinations and their corresponding trainable parameters in the performance of the edge LLM.

\textbf{RAG}: RAG consists of a retriever that is commonly based on max inner product search (MIPS) and a generator which usually is an LLM. The retriever gets the appropriate query-relevant information from user history data to formalize the final prompt \cite{lewis2020retrieval}. While this method does not consume resources to fine-tune the model, it requires saving all user history data embeddings for information retrieval. As user history data accumulates, the data embeddings can become a significant burden on the edge device \cite{qin2024robust}. In our experiments, we focus on the size of user history data and set all other hyperparameters to default, as shown in Appendix~\ref{subsec:Experimental_Settings}.

Our experiments investigate how different settings in each method can impact model performance and study which method can outperform the other under certain circumstances.

\subsection{Models}
\label{subsec:models}
In addition to the data and learning method, the model itself can be undoubtedly important to the entire edge LLM framework. Under the constraints of edge devices, only the model with a certain size can be deployed. There are two types of models that can satisfy such constraints, either small-scale uncompressed models or models compressed from large-scale models. In our experiments, we examine both types of models.

\textbf{Uncompressed models}: Their performance can mostly related to their initial architectures and how they are trained. While they may not contain certain pre-trained knowledge due to the limitation of size, their performance will not risk being deteriorated by the compression methods. For such models, we mainly investigate Pythia \cite{biderman2023pythia}, OPT \cite{zhang2022opt}, Llama \cite{touvron2023llama}, Gemma \cite{team2024gemma}, and StableLM \cite{bellagente2024stable} series of models. To fit them into the corresponding edge device, we select each model with different weight sizes. Additionally, we profile these models under the edge environment settings to ensure that their peak resource usage will not exceed the resource limitation of the edge devices they are deployed on. The detailed model information along with their corresponding edge device information can be found in Appendix~\ref{subsec:Experimental_Settings}, Table~\ref{tab:model_data}. 

\textbf{Compressed models}: Other than their initial architectures and pre-training, the compression methods can also largely impact the model performance. There are three mainstream compression methods, including quantization \cite{rokh2022comprehensive}, pruning \cite{liu2018rethinking}, and knowledge distillation \cite{gou2021knowledge}. Model compression normally squeezes a large and pre-trained model into a smaller model. While each method can have certain advantages, the past works \cite{polino2018model} mainly study such advantages for cloud-deployed LLMs, and it is not clear which one works best for compressing LLMs for edge devices. Among the existing compressed models, we select Llama, Mistral \cite{jiang2023mistral}, Synthia \cite{Synthia-70B-v1.2}, Gemma, and StableLM quantized by GPTQ \cite{frantar2022gptq} as the quantization models, Sheared-Llama \cite{xia2023sheared} as the pruning models, and Phi \cite{gunasekar2023textbooks} as the knowledge distillation models. Each series of the model contains various sizes, which allows us to deploy them on different edge devices and investigate their performance under a wide range of edge devices. The detailed model compression methods can be found in Appendix~\ref{subsec:Model_Compression}



==> 5_discuss.tex <==

    


% \section{Discussion \dcheng{and Guidebook of Edge LLMs} \rqin{[section 4 is about observation and analysis, section 5 is guidebook]}}
% \label{sec:discuss}

    

% \dcheng{In this section, we summarize the previous section's findings and provide the guidebook for choosing appropriate optimizations of edge LLMs to the readers.}

% \subsection{Task difficulty can impact Edge LLM design}
% \rqin{Here we need to talk about how the task difficulty, as an external factor, can impact the performance and learning effectiveness. We need to add it into our guidebook}

% \dcheng{We should choose the LLM based on the difficulty of the downstream task. For classification tasks, small LLMs with PEFT are preferred over larger ones when the task is simple. As the task difficulty increases, we should gradually shift to larger LLMs with RAG. PEFT fine-tuning on large models is generally not recommended on edge devices. While they potentially reach better accuracy compared to RAG, their ability to adapt to downstream tasks with limited data due to time and resource constraints remains uncertain. When the task's difficulty cannot be assessed, Phi models with PEFT fine-tuning are usually a good starting point. }

% \dcheng{On the other hand, for summarization tasks, larger LLMs are preferred due to the requirement for their inherent semantic understanding abilities. Similar to classification tasks, fine-tuning might reach better performance, but it is less stable than RAG.}

% \subsection{PEFT: Trade-off between model size, data size, and optimization \dcheng{methods}}
% \rqin{In this section, we are going to discuss the trade-off between these three things. Provide some statements with explanation and support.}

% \rqin{[model is the most important factor]}

% \dcheng{I kind of covered the questions in the previous subsection. Maybe change this section to a discussion of optimization methods}

% \dcheng{In this section, we discuss the different behaviors of three optimization methods: quantization, distillation, and pruning. Through experiments, we see that distillation methods have a stably good performance, quantization through GPTQ achieves the best performance if the hyperparameters are tuned correctly, but tuning the PEFT hyperparameters sometimes is not feasible for practical usage. Pruning has high potential in putting large models into edge devices, but they do not support fine-tuning, which hinders their usage for downstream tasks.}
% \begin{itemize}
%     \item Question 1: Within \textbf{limited} space, bigger data or bigger model, which one is better?
%     \item Question 2: What is the upper and lower bound? (Need learning curves.)
% \end{itemize}




% \subsection{Time, workload, and efficiency}
% \rqin{When we further discuss the trade-off, we brought up the more practical question towards edge devices: given the usage of edge devices like phone, how much time can the user bear for the Edge LLM to learn. Learning can consume energy and computational power. Such a high workload prevents other programs to properly execute. This leads to the importance of efficiency, which is much more critical in edge device than cluster computing.}

% \begin{itemize}[leftmargin=*]
%     \item \rqin{[Finding 1]: On edge devices, a larger model does not conduct better learning performance while it consumes more resources.} \dcheng{Chinchilla's scaling law \cite{hoffmann2022training} states that the pre-training data size should be proportional to the model's size. We observe the same scaling law on edge devices when fine-tuning LLMs for downstream tasks. Larger LLMs need more data to adapt to downstream tasks, but because of the time constraints on edge devices, larger LLMs in fact could only process less training data compared to smaller models. This means that unless we need to leverage larger LLM's inherent semantic understanding abilities, smaller models are preferred on the edge when fine-tuning time is insufficient.}
%     \item \dcheng{[Finding 2]: Longer time fine-tuning does not always yield the best results for downstream tasks. We see that lots of tutorials on fine-tuning LLMs do not set a validation dataset (this is arguably also a very common approach for the LLM community), but their focus is on larger models. While such an approach works for larger cloud LLMs, it is not suitable for edge LLMs. During experiments, the performance of most models is not monotonically increasing, and we have found that smaller LLMs have a non-zero possibility of overfitting to training data, especially when the task is relatively easy. We warn the community about this finding and urge the usage of a validation dataset for early stopping when fine-tuning small LLMs.}
%     \item \rqin{[no need to grid search for LoRA, any setting can do, based on our experiments, we suggest to fix LoRA setting as ...]}
% \end{itemize}

% \subsection{\dcheng{Future directions of developing edge LLMs} \rqin{[can merge with conclusion]}}


==> tables/table_stats_tasks.tex <==
\begin{table}[t]
\centering
\caption{[Insert your caption here]}
{\fontsize{7.5}{11}\selectfont % Set font size to 6pt with a line spacing of 7.2pt
\begin{tabularx}{\textwidth}{>{\hsize=1\hsize\centering\arraybackslash}X>{\hsize=1\hsize\centering\arraybackslash}X>{\hsize=0.5\hsize\centering\arraybackslash}X>{\hsize=0.8\hsize\centering\arraybackslash}X>{\hsize=1\hsize\centering\arraybackslash}X} % Centering text in each column
\toprule
Task & Type & Dataset & Difficulty &  Metric \\ % Add column headers
\midrule
Citation Choosing   & Classification    &  LaMP-1 &   0.4975   & Accuracy, F1  \\
Movie Tagging       & Classification    &  LaMP-2 &   0.3436   & Accuracy, F1  \\
Product Rating      & Classification    &  LaMP-3 &   0.6472   & Accuracy, F1  \\
New Headline        & Generation        &  LaMP-4 &   0.1460   & ROUGE-1/L  \\
Scholarly Title     & Generation        &  LaMP-5 &   0.3123   & ROUGE-1/L  \\
Email Subject       & Generation        &  LaMP-6 &   0.3475   & ROUGE-1/L  \\
Tweet Paraphrase    & Generation        &  LaMP-7 &   0.2385   & ROUGE-1/L  \\
\bottomrule
\end{tabularx}
} % End of font size group
\label{tab:stats_tasks}
\end{table}

